Role of Externally Provided Randomness in Stochastic Teams and Zero-sum Team Games

Stochastic team decision problem is extensively studied in literature and the existence of optimal solution is obtained in recent literature. The value of information in statistical problem and decision theory is classical problem. Much of earlier does not qualitatively describe role of externally provided private and common randomness in stochastic team problem and team vs team zero sum game. In this paper, we study the role of extrenally provided private or common randomness in stochastic team decision. We make observation that the randomness independent of environment does not benefit either team but randomness dependent on environment benefit teams and decreases the expected cost function. We also studied LQG team game with special information structure on private or common randomness. We extend these study to problem team vs team zero sum game. We show that if a game admits saddle point solution, then private or common randomness independent of environment does not benefit either team. We also analyze the scenario when a team with having more information than other team which is dependent on environment and game has saddle point solution, then team with more information benefits. This is also illustrated numerically for LQG team vs team zero sum game. Finally, we show for discrete team vs team zero sum game that private randomness independent of environment benefits team when there is no saddle point condition. Role of common randomness is discussed for discrete game.

==> macros-math.tex <==

\newtheorem{theorem}{Theorem}[section]
\newtheorem{assumption}{Assumption}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{conjecture}{Conjecture}[section]
\newtheorem{claim}[theorem]{Claim}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{prop}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{cor}[theorem]{Corollary}
\newtheorem{result}[theorem]{Result}
\newtheorem{definition}{Definition}[section]
\newenvironment{keywords}{{\noindent \bf Keywords:}}{}
\newenvironment{amsclass}{{\noindent \bf AMS Subject Classification:}}{}

\newenvironment{proofarg}[1][]{{\noindent \bf Proof #1: }}{\hfill \qed\vspace{6pt}}
\newenvironment{proof}[1][]{{\noindent \bf Proof #1: }}{\hfill \qed \vspace{3pt}\\ }
\newenvironment{examplee}{{\noindent \bf Example}}{\hfill $\square$\hspace{-4.5pt}\vspace{6pt}}
\newcounter{example}
\renewcommand{\theexample}{\thesection.\arabic{example}}
\newenvironment{examplec}[1][]{\refstepcounter{example}
\par\medskip \noindent%
   \textbf{Example~\theexample. #1} \rmfamily}{\hfill $\square$   \hspace{-4.5pt} \vspace{6pt}}


\newcounter{remark}
\renewcommand{\theremark}{\thesection.\arabic{remark}}
\newenvironment{remarkc}[1][]{\refstepcounter{remark}
\par\medskip \noindent%
   \textbf{Remark~\theremark. #1} \rmfamily}{\hfill $\square$   \hspace{-4.5pt} \vspace{6pt}}
\newenvironment{remark}{\vspace{.8\baselineskip}{\noindent \bf Remark : }}{\hfill $\square$\hspace{-4.5pt} \vspace{3pt}}
%\input{/home/ankur/latexfiles/algorithm2e.sty}
%  \def\proof{\penalty 25\noindent{\bf Proof.}\nobreak\hskip 1em\ignorespaces}
\def\noproof{\hspace{1em}\blackslug}
\def\mm#1{\hbox{$#1$}}                 % math mode
\def\mtx#1#2{\renewcommand{\arraystretch}{1.2}%
    \left(\! \begin{array}{#1}#2\end{array}\! \right)}



\def\shiftpar#1{\noindent \hangindent#1}
\newenvironment{indentpar}[1]%
{\begin{list}{}%
         {\setlength{\leftmargin}{#1}}%
         \item[]%
}
{\end{list}}




		% -- Environments --
		\def\bsp{\begin{split}}
		\def\beq{\begin{eqnarray}}
		\def\bal{\begin{align*}}
		\def\bc{\begin{center}}
		\def\be{\begin{enumerate}}
		\def\bi{\begin{itemize}}
		\def\bs{\begin{small}}
		\def\bS{\begin{slide}}
		\def\ec{\end{center}}
		\def\ee{\end{enumerate}}
		\def\ei{\end{itemize}}
		\def\es{\end{small}}
		\def\eS{\end{slide}}
		\def\eeq{\end{eqnarray}}
		\def\eal{\end{align*}}
		\def\esp{\end{split}}
		\def\qed{ \vrule height7.5pt width7.5pt depth0pt}  %width4.17pt depth0pt} 
		\def\problemlarge#1#2#3#4{\fbox
		 {\begin{tabular*}{.88\textwidth}
			{@{}l@{\extracolsep{\fill}}l@{\extracolsep{6pt}}l@{\extracolsep{\fill}}c@{}}
				#1 & $\minimize{#2}$ & $#3$ & $ $ \\[5pt]
					 & $\subject\ $    & $#4$ & $ $
			\end{tabular*}}
			}
		\def\problemsuperlarge#1#2#3#4{\fbox
           {\tiny      {\begin{tabular*}{.95\textwidth}
                        {@{}l@{\extracolsep{\fill}}l@{\extracolsep{6pt}}l@{\extracolsep{\fill}}c@{}}
                              #1 & $\minimize{#2}$ &  $#3$ & $ $ \\[12pt]
                                         & $\subject\ $    & $#4$ & $ $
                        \end{tabular*}} }
                        }
	\def\maxproblemlarge#1#2#3#4{\fbox
		 {\begin{tabular*}{1.05\textwidth}
			{@{}l@{\extracolsep{\fill}}l@{\extracolsep{6pt}}l@{\extracolsep{\fill}}c@{}}
				#1 & $\maximize{#2}$ & $#3$ & $ $ \\[5pt]
					 & $\subject\ $    & $#4$ & $ $
			\end{tabular*}}
			}
	\def\maxproblemsmall#1#2#3#4{\fbox
		 {\begin{tabular*}{0.55\textwidth}
			{@{}l@{\extracolsep{\fill}}l@{\extracolsep{6pt}}l@{\extracolsep{\fill}}c@{}}
				#1 & $\maximize{#2}$ & $#3$ & $ $ \\[5pt]
					 & $\subject\ $    & $#4$ & $ $
			\end{tabular*}}
			}



\newcommand{\boxedeqnnew}[2]{\vspace{12pt}
 \noindent\framebox[\textwidth]{\begin{tabular*}{\textwidth}{p{.8\textwidth}p{.15\textwidth}}
                             \hspace{.05 \textwidth}    #1 & \raggedleft #2
                                \end{tabular*}
}\vspace{12pt}
 }

\newcommand{\boxedeqn}[3]{\vspace{-.2in}
\begin{center}
  \fbox{%
      \begin{minipage}{#2 \textwidth}%
      \begin{equation}#1 #3 \end{equation}%
      \end{minipage}%
    }%
    \end{center}
}
\newcommand{\boxedeqnsmall}[6]{\vspace{12pt}
 \noindent\framebox[#3 \textwidth]{\begin{tabular*}{#3 \textwidth}{p{#5 \textwidth }p{#6 \textwidth }}
                               \hspace{#4 \textwidth}  #1 & \raggedleft #2
                                \end{tabular*}
}\vspace{12pt}
 }


\newcommand{\anybox}[2]
{\fbox{
\begin{minipage}
\begin{tabular*}{#2 \texwidth}{l}
#1
\end{tabular*}
\end{minipage}
}}

		\def\problemsmall#1#2#3#4{\fbox
		 {\begin{tabular*}{0.48\textwidth}
			{@{}l@{\extracolsep{\fill}}l@{\extracolsep{6pt}}l@{\extracolsep{\fill}}c@{}}
				#1 & $\minimize{#2}$ & $#3$ & $ $ \\[5pt]
					 & $\subject\ $    & $#4$ & $ $
			\end{tabular*}}
			}

		\def\problem#1#2#3#4{\fbox
		 {\begin{tabular*}{0.80\textwidth}
			{@{}l@{\extracolsep{\fill}}l@{\extracolsep{6pt}}l@{\extracolsep{\fill}}c@{}}
				#1 & $\minimize{#2}$ & $#3$ & $ $ \\[5pt]
					 & $\subject\ $    & $#4$ & $ $
			\end{tabular*}}
			}
\def\maxproblem#1#2#3#4{\fbox
		 {\begin{tabular*}{0.80\textwidth}
			{@{}l@{\extracolsep{\fill}}l@{\extracolsep{6pt}}l@{\extracolsep{\fill}}c@{}}
				#1 & $\maximize{#2}$ & $#3$ & $ $ \\[5pt]
					 & $\subject\ $    & $#4$ & $ $
			\end{tabular*}}
			}

\def\maxxproblem#1#2#3#4{\fbox
		 {\begin{tabular*}{1.1\textwidth}
			{@{}l@{\extracolsep{\fill}}l@{\extracolsep{6pt}}l@{\extracolsep{\fill}}c@{}}
				#1 & $\maximize{#2}$ & $#3$ & $ $ \\[5pt]
					 & $\subject\ $    & $#4$ & $ $
			\end{tabular*}}
			}

\def\unconmaxproblem#1#2#3#4{\fbox
		 {\begin{tabular*}{0.95\textwidth}
			{@{}l@{\extracolsep{\fill}}l@{\extracolsep{6pt}}l@{\extracolsep{\fill}}c@{}}
				#1 & $\maximize{#2}$ & $#3$ & $ $ \\[5pt]
			\end{tabular*}}
			}

\def\unconproblem#1#2#3#4{\fbox
		 {\begin{tabular*}{0.95\textwidth}
			{@{}l@{\extracolsep{\fill}}l@{\extracolsep{6pt}}l@{\extracolsep{\fill}}c@{}}
				#1 & $\minimize{#2}$ & $#3$ & $ $ \\[5pt]
			\end{tabular*}}
			}
	\def\cpproblem#1#2#3#4{\fbox
		 {\begin{tabular*}{0.95\textwidth}
			{@{}l@{\extracolsep{\fill}}l@{\extracolsep{6pt}}l@{\extracolsep{\fill}}c@{}}
				#1 & & $#4 $ 
			\end{tabular*}}}
	\def\cp2problem#1#2#3#4{\fbox
		 {\begin{tabular*}{0.9\textwidth}
			{@{}l@{\extracolsep{\fill}}l@{\extracolsep{6pt}}l@{\extracolsep{\fill}}c@{}}
				#1 & & $#4 $ 
			\end{tabular*}}}
\def\z{\phantom 0}
\newcommand{\pmat}[1]{\begin{pmatrix} #1 \end{pmatrix}}
		\newcommand{\botline}{\vspace*{-1ex}\hrulefill}
		\renewcommand{\emph}[1]{\textbf{#1}}
		\newcommand{\clin}[2]{c\L(#1,#2)}
		\newcommand{\dlin}[2]{d\L(#1,#2)}
		\newcommand{\Fbox}[1]{\fbox{\quad#1\quad}}
		\newcommand{\mcol}[3]{\multicolumn{#1}{#2}{#3}}
		\newcommand{\assign}{\ensuremath{\leftarrow}}
		\newcommand{\ssub}[1]{\mbox{\scriptsize #1}}
		\def\bkE{{\rm I\kern-.17em E}}
		\def\bk1{{\rm 1\kern-.17em l}}
		\def\bkD{{\rm I\kern-.17em D}}
		\def\bkR{{\rm I\kern-.17em R}}
		\def\bkP{{\rm I\kern-.17em P}}
		
		\def\bkZ{{\bf{Z}}}
		\def\bkI{{\bf{I}}}

\def\boldp{\boldsymbol{p}}
\def\boldy{\boldsymbol{y}}


\newcommand {\beeq}[1]{\begin{equation}\label{#1}}
\newcommand {\eeeq}{\end{equation}}
\newcommand {\bea}{\begin{eqnarray}}
\newcommand {\eea}{\end{eqnarray}}
\newcommand{\mb}[1]{\mbox{\boldmath $#1$}}
\newcommand{\mbt}[1]{\mbox{\boldmath $\tilde{#1}$}}
\newcommand{\mbs}[1]{{\mbox{\boldmath \scriptsize{$#1$}}}}
\newcommand{\mbst}[1]{{\mbox{\boldmath \scriptsize{$\tilde{#1}$}}}}
\newcommand{\mbss}[1]{{\mbox{\boldmath \tiny{$#1$}}}}
\newcommand{\dpv}{\displaystyle \vspace{3pt}}
\def\texitem#1{\par\smallskip\noindent\hangindent 25pt
               \hbox to 25pt {\hss #1 ~}\ignorespaces}
\def\smskip{\par\vskip 7pt}
%\def\example{{\bf Example :\ }}
\def\st{\mbox{subject to}}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "report"
%%% End: 


==> macros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%        macros.tex                  %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{amsmath, amssymb, xspace}
\usepackage{epsfig}
\usepackage{longtable}
\usepackage{color}
\usepackage{mathrsfs}
\usepackage{subfig}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 	bb, bf and bk
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\Zbb{{\mathbb{Z}}}
\def\Cbb{{\mathbb{C}}}
\def\Nbb{{\mathbb{N}}}
\def\Fbb{{\mathbb{F}}}
\def\Prob{\mathbb{P}}
\def\Ebb{\mathbb{E}}
\def\Gbf{{\bf G}}
\def\Cbf{{\bf C}}
\def\Bbf{{\bf B}}
\def\Dbf{{\bf D}}
\def\Wbf{{\bf W}}
\def\Gbf{{\bf G}}
\def\Cbf{{\bf C}}
\def\Bbf{{\bf B}}
\def\Wbf{{\bf W}}
\def\Mbf{{\bf M}}
\def\Nbf{{\bf N}}

\def\Mbf{{\bf M}}
\def\Nbf{{\bf N}}
\def\Ibf{{\bf I}}
\def\bfzero{{\bf 0}}
\def\bfG{{\bf G}}
\def\bfR{{\bf R}}
\def\bfH{{\bf H}}
\def\bfL{{\bf L}}
\def\bfV{{\bf V}}
\def\bfE{{\bf E}}


\def\bfA{{\bf A}}
\def\bfU{{\bf U}}
\def\bfC{{\bf C}}
\def\bfone{{\bf 1}}
\def\bfe{{\bf e}}
\def\t{^\top}
\def\th{^{\rm th}}
\def\bfm{{\bf m}}


\def\bkE{{\rm I\kern-.17em E}}
\def\bk1{{\rm 1\kern-.17em l}}
\def\bkD{{\rm I\kern-.17em D}}
\def\bkR{{\rm I\kern-.17em R}}
\def\bkP{{\rm I\kern-.17em P}}
\def\bkN{{\mathbb{N}}}
\def\bkZ{{\bf{Z}}}
\def\bkE{{\rm I\kern-.17em E}}
\def\bk1{{\rm 1\kern-.17em l}}
\def\bkD{{\rm I\kern-.17em D}}
\def\bkR{{\rm I\kern-.17em R}}
\def\bkP{{\rm I\kern-.17em P}}
		\def\bkE{{\rm I\kern-.17em E}}
		\def\bk1{{\rm 1\kern-.17em l}}
		\def\bkD{{\rm I\kern-.17em D}}
		\def\bkR{{\rm I\kern-.17em R}}
		\def\bkP{{\rm I\kern-.17em P}}
		\def\bkY{{\bf \kern-.17em Y}}
		\def\bkZ{{\bf \kern-.17em Z}}
		\def\bkC{{\bf  \kern-.17em C}}



%%%%%%%%%%%%%%%%%%%%%%%%
% 	scr and cal
%%%%%%%%%%%%%%%%%%%%%%%%%
\def\Escr{\mathcal{E}}
\def\Fscrhat{\widehat{\Fscr}}
\def\Epec{{\mathscr{E}}}
\def\Xscr{\mathcal{X}}
\def\Yscr{\mathcal{Y}}
\def\Hcal{\mathcal{H}}
\def\Gcal{\mathcal{G}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Math italic and calligraphic fonts
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\Deltait{{\mit \Delta}}
\def\Deltabar{{\bar \Delta}}
\def\Gammait{{\mit \Gamma}}
\def\Lambdait{{\mit \Lambda}}
\def\Sigmait{{\mit \Sigma}}
\def\Lambarit{\skew5\bar{\mit \Lambda}}
\def\Omegait{{\mit \Omega}}
\def\Omegaitbar{\skew5\bar{\mit \Omega}}
\def\Thetait{{\mit \Theta}}
\def\Piitbar{\skew5\bar{\mit \Pi}}
\def\Piit{{\mit \Pi}}
\def\Phiit{{\mit \Phi}}

\def\Ksf{{\sf K}}
\def\Dsf{{\sf D}}
\def\Isf{{\sf I}}
\def\Nsf{{\sf N}}
\def\Csf{{\sf C}}

\def\Ascr{{\cal A}}
\def\Bscr{{\cal B}}
\def\Fscr{{\cal F}}
\def\Dscr{{\cal D}}
\def\Iscr{{\cal I}}
\def\Jscr{{\cal J}}
\def\Lscr{{\cal L}}
\def\Hscr{{\cal H}}
\def\Mscr{{\cal M}}
\def\Tscr{{\cal T}}
\def\lscr{\ell}
\def\lscrbar{\ellbar}
\def\Oscr{{\cal O}}
\def\Pscr{{\cal P}}
\def\Qscr{{\cal Q}}
\def\Sscr{{\cal S}}
\def\Sscrhat{\widehat{\mathcal{S}}}
\def\Uscr{{\cal U}}
\def\Vscr{{\cal V}}
\def\Wscr{{\cal W}}
\def\Mscr{{\cal M}}
\def\Nscr{{\cal N}}
\def\Rscr{{\cal R}}
\def\Gscr{{\cal G}}
\def\Cscr{{\cal C}}
\def\Zscr{{\cal Z}}
\def\Kscr{{\cal K}}

\def\MINOS{{\small MINOS}}
\def\NPSOL{{\small NPSOL}}
\def\QPSOL{{\small QPSOL}}
\def\LUSOL{{\small LUSOL}}
\def\LSSOL{{\small LSSOL}}


\def\supp{{\rm supp}}
\def\aur{\;\textrm{and}\;}
\def\where{\;\textrm{where}\;}
\def\eef{\;\textrm{if}\;}
\def\ow{\;\textrm{otherwise}}
\def\del{\partial}
\def\non{\nonumber}
\def\OPT{{\rm OPT}}
\def\SOL{{\rm SOL}}
\def\VI{{\rm VI}}
\def\VIs{{\rm VIs}}
\def\QVI{{\rm QVI}}
\def\QVIs{{\rm QVIs}}
\def\LCP{{\rm LCP}}
\def\GNE{{\rm GNE}}
\def\VE{{\rm VE}}
\def\GNEs{{\rm GNEs}}
\def\VEs{{\rm VEs}}
\def\SYS{{\rm (SYS)}}
\def\bfI{{\bf I}}
\let\forallnew\forall
\renewcommand{\forall}{\forallnew\ }
\let\forall\forallnew


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%	miscellaneous
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\newcommand{\mlmfg}{multi-leader multi-follower game\@\xspace}
\newcommand{\mlmfgs}{multi-leader multi-follower games\@\xspace}
\def\ds{\displaystyle}

\newcommand{\scg}{shared-constraint game\@\xspace} %%% i.e.,
\newcommand{\scgs}{shared-constraint games\@\xspace}
\newcommand{\Scgs}{Shared-constraint games\@\xspace}

\def\b12{(\beta_1,\beta_2)}
\def\Epec{{\mathscr{E}}}

\def\fnatt{\widetilde{\bf F}^{\rm nat}}
\def\gnat{{\bf G}^{\rm nat}}
\def\jnat{{\bf J}^{\rm nat}}


\def\fnat{{\bf F}^{\textrm{nat}}}
\def\xref{x^{\textrm{ref}}}
\def\zref{z^{\textrm{ref}}}
\def\intt{{\textrm{int}}} 
\def\fnatt{\widetilde{\bf F}^{\textrm{nat}}}
\def\gnat{{\bf G}^{\textrm{nat}}}
\def\jnat{{\bf J}^{\textrm{nat}}}
\def\sthat{\ {\rm such\ that}\ }
\def\eig{{\rm eig}}
\def\eigmax{\eig_{\max}}
\def\eigmin{\eig_{\min}}
\def\mi{^{-i}}
\def\indep{\perp\!\!\!\!\perp}
\def\modulo{{\rm\ mod\,}}
\newcommand{\I}[1]{\mathbb{I}_{\{#1\}}}
\def\fnat{{\bf F}^{\rm nat}}
\def\fnor{{\bf F}^{\textrm{nor}}}
\def\subject{\hbox{\rm subject to}}
\newcommand{\Real}{\ensuremath{\mathbb{R}}}
\newcommand{\inv}{^{-1}}
\newcommand{\dom}{\mathrm{dom}}
\def\asn{\buildrel{n}\over\rightarrow}
\def\xref{x^{\rm ref}}
\def\as{{\rm a.s.}}
\def\reff{^{\rm ref}}
\def\limn{\ds \lim_{n \rightarrow \infty}}
\def\limt{\ds \lim_{t \rightarrow \infty}}
\def\sumn{\ds \sum_{n=0}^{\infty}}
\def\asst{\buildrel{t}\over\rightarrow}
\def\asn{\buildrel{n}\over\rightarrow}
\def\inp{\buildrel{p.}\over\rightarrow}
\def\ind{{\rm ind}}
\def\Gr{{\rm graph}}
\def\cross{\scriptscriptstyle\times}
\def\cond{\hbox{\rm cond}}
\def\det{\mathop{\hbox{\rm det}}}
\def\diag{\mathop{\hbox{\rm diag}}}
\def\diam{\mathop{\hbox{\rm diam}}}
\def\dim{\mathop{\hbox{\rm dim}}}  
\def\exp{\mathop{\hbox{\rm exp}}}  
\def\In{\mathop{\hbox{\it In}\,}}
\def\boundary{\mathop{\hbox{\rm bnd}}}
\def\interior{\mathop{\hbox{\rm int}}}
\def\Null{\mathop{\hbox{\rm null}}}
\def\rank{\mathop{\hbox{\rm rank}}}
\def\op{\mathop{\hbox{\rm op}}}
\def\Range{\mathop{\hbox{\rm range}}}
%\def\range{\mathop{\hbox{\rm range}}}
\def\range{{\rm range}}
\def\sign{\mathop{\hbox{\rm sign}}}
\def\sgn{\mathop{\hbox{\rm sgn}}}
\def\Span{\mbox{\rm span}}
\def\intt{{\rm int}}
\def\trace{\mathop{\hbox{\rm trace}}}
\def\drop{^{\null}}
%\def\etal{{\em et al.\ }}  %%% e.g., Gill \etal (1986)
\def\float{fl}
\def\grad{\nabla}
\def\Hess{\nabla^2}
\def\half  {{\textstyle{1\over 2}}}
\def\third {{\textstyle{1\over 3}}}
\def\fourth{{\textstyle{1\over 4}}}
\def\sixth{{\textstyle{1\over 6}}}
\def\Nth{{\textstyle{1\over N}}}
\def\nth{{\textstyle{1\over n}}}
\def\mth{{\textstyle{1\over m}}}
\def\invsq{^{-2}}
\def\limk{\lim_{k\to\infty}}
\def\limN{\lim_{N\to\infty}}
\def\conv{\textrm{conv}\:}
\def\cl{\mbox{cl}\:}
\def\xint{{x_{\rm int}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%	Hat and bar
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
\def\abar{\skew3\bar a}
\def\ahat{\skew2\widehat a}
\def\atilde{\skew2\widetilde a}
\def\Abar{\skew7\bar A}
\def\Ahat{\widehat A}
\def\Atilde{\widetilde A}
\def\bbar{\skew3\bar b}
\def\bhat{\skew2\widehat b}
\def\btilde{\skew2\widetilde b}
\def\Bbar{\bar B}
\def\Bhat{\widehat B}
\def\cbar{\skew5\bar c}
\def\chat{\skew3\widehat c}
\def\ctilde{\widetilde c}
\def\Cbar{\bar C}
\def\Chat{\widehat C}
\def\Ctilde{\widetilde C}
\def\dbar{\bar d}
\def\dhat{\widehat d}
\def\dtilde{\widetilde d}
\def\Dbar{\bar D}
\def\Dhat{\widehat D}
\def\Dtilde{\widetilde D}
\def\ehat{\skew3\widehat e}
\def\ebar{\bar e}
\def\Ebar{\bar E}
\def\Ehat{\widehat E}
\def\fbar{\bar f}
\def\fhat{\widehat f}
\def\ftilde{\widetilde f}
\def\Fbar{\bar F}
\def\Fhat{\widehat F}
\def\gbar{\skew{4.3}\bar g}
\def\ghat{\skew{4.3}\widehat g}
\def\gtilde{\skew{4.5}\widetilde g}
\def\Gbar{\bar G}
\def\Ghat{\widehat G}
%\def\hbar{\skew{4.2}\bar h}
\def\hhat{\skew2\widehat h}
\def\htilde{\skew3\widetilde h}
\def\Hbar{\skew5\bar H}
\def\Hhat{\widehat H}
\def\Htilde{\widetilde H}
\def\Ibar{\skew5\bar I}
\def\Itilde{\widetilde I}
\def\Jbar{\skew6\bar J}
\def\Jhat{\widehat J}
\def\Jtilde{\widetilde J}
\def\kbar{\skew{4.4}\bar k}
\def\Khat{\widehat K}
\def\Kbar{\skew{4.4}\bar K}
\def\Ktilde{\widetilde K}
\def\ellbar{\bar \ell}
\def\lhat{\skew2\widehat l}
\def\lbar{\skew2\bar l}
\def\Lbar{\skew{4.3}\bar L}
\def\Lhat{\widehat L}
\def\Ltilde{\widetilde L}
\def\mbar{\skew2\bar m}
\def\mhat{\widehat m}
\def\Mbar{\skew{4.4}\bar M}
\def\Mhat{\widehat M}
\def\Mtilde{\widetilde M}
\def\Nbar{\skew{4.4}\bar N}
\def\Ntilde{\widetilde N}
\def\nbar{\skew2\bar n}
\def\pbar{\skew2\bar p}
%\def\phat{\skew2\widehat p}
\def\phat{\skew2\widehat p}
\def\ptilde{\skew2\widetilde p}
\def\Pbar{\skew5\bar P}
\def\phibar{\skew5\bar \phi}
\def\Phat{\widehat P}
\def\Ptilde{\skew5\widetilde P}
\def\qbar{\bar q}
\def\qhat{\skew2\widehat q}
\def\qtilde{\widetilde q}
\def\Qbar{\bar Q}
\def\Qhat{\widehat Q}
\def\Qtilde{\widetilde Q}
\def\rbar{\skew3\bar r}
\def\rhat{\skew3\widehat r}
\def\rtilde{\skew3\widetilde r}
\def\Rbar{\skew5\bar R}
\def\Rhat{\widehat R}
\def\Rtilde{\widetilde R}
\def\sbar{\bar s}
\def\shat{\widehat s}
\def\stilde{\widetilde s}
\def\Shat{\widehat S}
\def\Sbar{\skew2\bar S}
\def\tbar{\bar t}
\def\ttilde{\widetilde t}
\def\that{\widehat t}
\def\Tbar{\bar T}
\def\That{\widehat T}
\def\Ttilde{\widetilde T}
\def\ubar{\skew3\bar u}
\def\uhat{\skew3\widehat u}
\def\utilde{\skew3\widetilde u}
\def\Ubar{\skew2\bar U}
\def\Uhat{\widehat U}
\def\Utilde{\widetilde U}
\def\vbar{\skew3\bar v}
\def\vhat{\skew3\widehat v}
\def\vtilde{\skew3\widetilde v}
\def\Vbar{\skew2\bar V}
\def\Vhat{\widehat V}
\def\Vtilde{\widetilde V}
\def\UBtilde{\widetilde {UB}}
\def\Utilde{\widetilde {U}}
\def\LBtilde{\widetilde {LB}}
\def\Ltilde{\widetilde {L}}
\def\wbar{\skew3\bar w}
\def\what{\skew3\widehat w}
\def\wtilde{\skew3\widetilde w}
\def\Wbar{\skew3\bar W}
\def\What{\widehat W}
\def\Wtilde{\widetilde W}
\def\xbar{\skew{2.8}\bar x}
\def\xhat{\skew{2.8}\widehat x}
\def\xtilde{\skew3\widetilde x}
\def\Xhat{\widehat X}
\def\ybar{\skew3\bar y}
\def\yhat{\skew3\widehat y}
\def\ytilde{\skew3\widetilde y}
\def\Ybar{\skew2\bar Y}
\def\Yhat{\widehat Y}
\def\zbar{\skew{2.8}\bar z}
\def\zhat{\skew{2.8}\widehat z}
\def\ztilde{\skew{2.8}\widetilde z}
\def\Zbar{\skew5\bar Z}
\def\Zhat{\widehat Z}
\def\Ztilde{\widetilde Z}


\def\vhat{{\hat v}}
\def\fhat{{\hat f}}
\def\xhat{{\hat x}}
\def\zhat{{\hat x}}
\def\phihat{{\widehat \phi}}
\def\xihat{{\widehat \xi}}
\def\betahat{{\widehat \beta}}
\def\psihat{{\widehat \psi}}
\def\thetahat{{\hat \theta}}
\def\Asubk{A\sub{\nthinsp k}}
\def\Bsubk{B\sub{\nthinsp k}}
\def\Fsubk{F\sub{\nmedsp k}}
\def\Gsubk{G\sub{\nthinsp k}}
\def\Hsubk{H\sub{\nthinsp k}}
\def\HsubB{H\sub{\nthinsp \scriptscriptstyle{B}}}
\def\HsubS{H\sub{\nthinsp \scriptscriptstyle{S}}}
\def\HsubBS{H\sub{\nthinsp \scriptscriptstyle{BS}}}
\def\Hz{H\sub{\nthinsp \scriptscriptstyle{Z}}}
\def\Jsubk{J\sub{\nmedsp k}}
\def\Psubk{P\sub{\nthiksp k}}
\def\Qsubk{Q\sub{\nthinsp k}}
\def\Vsubk{V\sub{\nmedsp k}}
\def\Vsubone{V\sub{\nmedsp 1}}
\def\Vsubtwo{V\sub{\nmedsp 2}}
\def\Ysubk{Y\sub{\nmedsp k}}
\def\Wsubk{W\sub{\nthiksp k}}
\def\Zsubk{Z\sub{\nthinsp k}}
\def\Zsubi{Z\sub{\nthinsp i}}

%%% Subscripts

\def\subfr{_{\scriptscriptstyle{\it FR}}}
\def\subfx{_{\scriptscriptstyle{\it FX}}}
\def\fr{_{\scriptscriptstyle{\it FR}}}
\def\fx{_{\scriptscriptstyle{\it FX}}}
\def\submax{_{\max}}
\def\submin{_{\min}}
\def\subminus{_{\scriptscriptstyle -}}
\def\subplus {_{\scriptscriptstyle +}}

\def\Ass{_{\scriptscriptstyle A}}
\def\Bss{_{\scriptscriptstyle B}}
\def\BSss{_{\scriptscriptstyle BS}}
\def\Css{_{\scriptscriptstyle C}}
\def\Dss{_{\scriptscriptstyle D}}
\def\Ess{_{\scriptscriptstyle E}}
\def\Fss{_{\scriptscriptstyle F}}
\def\Gss{_{\scriptscriptstyle G}}
\def\Hss{_{\scriptscriptstyle H}}
\def\Iss{_{\scriptscriptstyle I}}
\def\w{_w}
\def\k{_k}
\def\kp#1{_{k+#1}}
\def\km#1{_{k-#1}}
\def\j{_j}
\def\jp#1{_{j+#1}}
\def\jm#1{_{j-#1}}
\def\K{_{\scriptscriptstyle K}}
\def\L{_{\scriptscriptstyle L}}
\def\M{_{\scriptscriptstyle M}}
\def\N{_{\scriptscriptstyle N}}
\def\subb{\B}
\def\subc{\C}
\def\subm{\M}
\def\subf{\F}
\def\subn{\N}
\def\subh{\H}
\def\subk{\K}
\def\subt{_{\scriptscriptstyle T}}
\def\subr{\R}
\def\subz{\Z}
\def\O{_{\scriptscriptstyle O}}
\def\Q{_{\scriptscriptstyle Q}}
\def\P{_{\scriptscriptstyle P}}
\def\R{_{\scriptscriptstyle R}}
\def\S{_{\scriptscriptstyle S}}
\def\U{_{\scriptscriptstyle U}}
\def\V{_{\scriptscriptstyle V}}
\def\W{_{\scriptscriptstyle W}}
\def\Y{_{\scriptscriptstyle Y}}
\def\Z{_{\scriptscriptstyle Z}}

%%% Superscript stars

\def\superstar{^{\raise 0.5pt\hbox{$\nthinsp *$}}}
\def\SUPERSTAR{^{\raise 0.5pt\hbox{$*$}}}
\def\shrink{\mskip -7mu}  %%% Less space after \xstar if followed by , or .

\def\alphastar{\alpha\superstar}
\def\lamstar  {\lambda\superstar}
\def\lamstarT {\lambda^{\raise 0.5pt\hbox{$\nthinsp *$}T}}
\def\lambdastar{\lamstar}
\def\nustar{\nu\superstar}
\def\mustar{\mu\superstar}
\def\pistar{\pi\superstar}
\def\s{^*}

\def\cstar{c\superstar}
\def\dstar{d\SUPERSTAR}
\def\fstar{f\SUPERSTAR}
\def\gstar{g\superstar}
\def\hstar{h\superstar}
\def\mstar{m\superstar}
\def\pstar{p\superstar}
\def\sstar{s\superstar}
\def\ustar{u\superstar}
\def\vstar{v\superstar}
\def\wstar{w\superstar}
\def\xstar{x\superstar}
\def\ystar{y\superstar}
\def\zstar{z\superstar}

\def\Astar{A\SUPERSTAR}
\def\Bstar{B\SUPERSTAR}
\def\Cstar{C\SUPERSTAR}
\def\Fstar{F\SUPERSTAR}
\def\Gstar{G\SUPERSTAR}
\def\Hstar{H\SUPERSTAR}
\def\Jstar{J\SUPERSTAR}
\def\Kstar{K\SUPERSTAR}
\def\Mstar{M\SUPERSTAR}
\def\Ustar{U\SUPERSTAR}
\def\Wstar{W\SUPERSTAR}
\def\Xstar{X\SUPERSTAR}
\def\Zstar{Z\SUPERSTAR}

%%% bars, hats, tildes  (\skew4 is the default)
\def\del{\partial}
\def\psibar{\bar \psi}
\def\alphabar{\bar \alpha}
\def\alphahat{\widehat \alpha}
\def\alphatilde{\skew3\tilde \alpha}
\def\betabar{\skew{2.8}\bar\beta}
\def\betahat{\skew{2.8}\hat\beta}
\def\betatilde{\skew{2.8}\tilde\beta}
\def\ftilde{\skew{2.8}\tilde f}
\def\delbar{\bar\delta}
\def\deltilde{\skew5\tilde \delta}
\def\deltabar{\delbar}
\def\deltatilde{\deltilde}
\def\lambar{\bar\lambda}
\def\etabar{\bar\eta}
\def\gammabar{\bar\gamma}
\def\lamhat{\skew{2.8}\hat \lambda}
\def\lambdabar{\lambar}
\def\lambdahat{\lamhat}
\def\mubar{\skew3\bar \mu}
\def\muhat{\skew3\hat \mu}
\def\mutilde{\skew3\tilde\mu}
\def\nubar{\skew3\bar\nu}
\def\nuhat{\skew3\hat\nu}
\def\nutilde{\skew3\tilde\nu}
\def\Mtilde{\skew3\tilde M}
\def\omegabar{\bar\omega}
\def\pibar{\bar\pi}
\def\pihat{\skew1\widehat \pi}
\def\sigmabar{\bar\sigma}
\def\sigmahat{\hat\sigma}
\def\rhobar{\bar\rho}
\def\rhohat{\widehat\rho}
\def\taubar{\bar\tau}
\def\tautilde{\tilde\tau}
\def\tauhat{\hat\tau}
\def\thetabar{\bar\theta}
\def\xibar{\skew4\bar\xi}
\def\UBbar{\skew4\overline {UB}}
\def\LBbar{\skew4\overline {LB}}
\def\xdot{\dot{x}}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 	environments etc
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5




\def\ebox{\fbox{\begin{minipage}{1pt}
\hspace{1pt}\vspace{1pt}
\end{minipage}}} 
\newlength{\noteWidth}
\setlength{\noteWidth}{.75in}
\long\def\notes#1{\ifinner
{\tiny #1}
\else
\marginpar{\parbox[t]{\noteWidth}{\raggedright\tiny #1}}
\fi\typeout{#1}}
 \def\notes#1{\typeout{read notes: #1}} %uncomment for final version

\def\noproof{\hspace{1em}\blackslug}
\def\mm#1{\hbox{$#1$}}                 % math mode
\def\mtx#1#2{\renewcommand{\arraystretch}{1.2}%
    \left(\! \begin{array}{#1}#2\end{array}\! \right)}
			\newcommand{\mQ}{\mathcal{Q}}
\newcommand{\ie}{i.e.\@\xspace} %%% i.e.,
\newcommand{\eg}{e.g.\@\xspace} %%% e.g.,
\newcommand{\etal}{et al.\@\xspace} %%% e.g., Gill \etal (1986)
\newcommand{\Matlab}{\textsc{Matlab}\xspace}
% Scientific Notation (E)
\newcommand{\e}[2]{{\small e}$\scriptstyle#1$#2}
% Miscellaneous items
%\renewcommand{\vec}[1]{\ensuremath{\mathbf{#1}}}  %requires amsmath package
\newcommand{\abs}[1]{\ensuremath{|#1|}}
\newcommand{\minimize}[1]{\displaystyle\minim_{#1}}
\newcommand{\minimum}[1]{\displaystyle\minum_{#1}}
\newcommand{\minim}{\mathop{\hbox{\rm minimize}}}
\newcommand{\minum}{\mathop{\hbox{\rm minimum}}}
\newcommand{\maximize}[1]{\displaystyle\maxim_{#1}}
\newcommand{\maxim}{\mathop{\hbox{\rm maximize}}}
\newcommand{\maximum}[1]{\displaystyle\maxum_{#1}}
\newcommand{\maxum}{\mathop{\hbox{\rm maximum}}}
\DeclareMathOperator*{\sbt}{subject\;to}
\newcommand{\twonorm}[1]{\norm{#1}_2}
\def\onenorm#1{\norm{#1}_1}
\def\infnorm#1{\norm{#1}_{\infty}}
\def\disp{\displaystyle}
\def\m{\phantom-}
\def\EM#1{{\em#1\/}}
\def\ur{\mbox{\bf u}}
\def\FR{I\!\!F}
\def\Complex{I\mskip -11.3mu C}
\def\sp{\hspace{10pt}}
\def\eval#1#2{\left.#2\right|_{\alpha=#1}}
\def\tmat#1#2{(\, #1 \ \ #2 \,)}
\def\tmatt#1#2#3{(\, #1 \ \  #2 \ \  #3\,)}
\def\tmattt#1#2#3#4{(\, #1 \ \  #2 \ \  #3 \ \  #4\,)}
\def\mat#1#2{(\; #1 \quad #2 \;)}
\def\matt#1#2#3{(\; #1 \quad #2 \quad #3\;)}
\def\mattt#1#2#3#4{(\; #1 \quad #2 \quad #3 \quad #4\;)}
\def\blackslug{\hbox{\hskip 1pt \vrule width 4pt height 6pt depth 1.5pt
  \hskip 1pt}}
\def\boxit#1{\vbox{\hrule\hbox{\vrule\hskip 3pt
  \vbox{\vskip 3pt #1 \vskip 3pt}\hskip 3pt\vrule}\hrule}}
\def\mystrut{\vrule height10.5pt depth5.5pt width0pt}
\def\mod#1{|#1|}
\def\modd#1{\biggl|#1\biggr|}
\def\Mod#1{\left|#1\right|}
\def\normm#1{\biggl\|#1\biggr\|}
\def\norm#1{\|#1\|}
\def\spose#1{\hbox to 0pt{#1\hss}}
\def\sub#1{^{\null}_{#1}}
\def\text #1{\hbox{\quad#1\quad}}
\def\textt#1{\hbox{\qquad#1\qquad}}
\def\T{^T\!}
\def\ntext#1{\noalign{\vskip 2pt\hbox{#1}\vskip 2pt}}
\def\enddef{{$\null$}}
%%% Fixed-size glue, only for math mode


\def\pthinsp{\mskip  2   mu}    %           thin space
\def\pmedsp {\mskip  2.75mu}    %         medium space
\def\pthiksp{\mskip  3.5 mu}    %          thick space
\def\nthinsp{\mskip -2   mu}
\def\nmedsp {\mskip -2.75mu}
\def\nthiksp{\mskip -3.5 mu}

%%% Specially lowered subscripts (see \sub above)



%		\usepackage[ruled,vlined,boxed]{algorithm2e}
		%\setlength{\baselineskip}{24pt}
		%\setlength{\topmargin}     { 0.0in}    % One inch top margins
		%\setlength{\headsep}       {24.0pt}    % with Header
		%\setlength{\textheight}    { 8.5in}
		%\setlength{\textwidth}     { 6.5in}    % One inch side margins
		%\setlength{\oddsidemargin} { 0.0in}
		%\setlength{\evensidemargin}{ 0.0in}
		%\setlength{\marginparsep}  { 0.0pt}    % No Margin notes
		%\setlength{\marginparwidth}{ 0.0pt}
		%\pagestyle{headings}

%%%%%%%%%%%%%%%%%%%%%
%Colours
%%%%%%%%%%%%%%%%%%%%%
%\definecolor{violet}{rgb}{.5,0.0,.80}
%\def\violet{{ \color{violet} }}
%\definecolor{dgreen}{rgb}{0,0.5,0.0}



